Tensor feature hallucination for few-shot learning

Few-shot learning addresses the challenge of learning how to address novel tasks given not just limited supervision but limited data as well. An attractive solution is synthetic data generation. However, most such methods are overly sophisticated, focusing on high-quality, realistic data in the input space. It is unclear whether adapting them to the few-shot regime and using them for the downstream task of classification is the right approach. Previous works on synthetic data generation for few-shot classification focus on exploiting complex models, e.g. a Wasserstein GAN with multiple regularizers or a network that transfers latent diversities from known to novel classes. We follow a different approach and investigate how a simple and straightforward synthetic data generation method can be used effectively. We make two contributions, namely we show that: (1) using a simple loss function is more than enough for training a feature generator in the few-shot setting; and (2) learning to generate tensor features instead of vector features is superior. Extensive experiments on miniImagenet, CUB and CIFAR-FS datasets show that our method sets a new state of the art, outperforming more sophisticated few-shot data augmentation methods. The source code can be found at https://github.com/MichalisLazarou/TFH_fewshot.

==> tex/app.tex <==
\appendix

\section{Appendix}

\subsection{Dataset details}
\label{app:datasets}

\paragraph{\emph{mini}ImageNet}

This is a widely used few-shot image classification dataset~\cite{matchingNets, ravilstm}. It contains 100 randomly sampled classes from ImageNet~\cite{imagenet}. These 100 classes are split into 64 training (base) classes, 16 validation (novel) classes and 20 test (novel) classes. Each class contains 600 examples (images). We follow the commonly used split proposed in~\cite{ravilstm}.

\paragraph{CUB}

This is a fine-grained classification dataset consisting of 200 classes, each corresponding to a bird species. We follow the split defined by~\cite{closerlook, fewshotCUB}, with 100 training, 50 validation and 50 test classes. 

\paragraph{CIFAR-FS}

This dataset is derived from CIFAR-100~\cite{cifar100db}, consisting of 100 classes with 600 examples per class. We follow the split provided by~\cite{closerlook}, with 64 training, 16 validation and 20 test classes.

All images from all datasets are resized to $224 \times 224$ in a similar way to other data augmentation methods \cite{AFHN, semanticAugmentation, Ideme, VIFSL}

%------------------------------------------------------------------------------
 
\subsection{Implementation details}
\label{app:implementations}

Our implementations are based on PyTorch \cite{pytorch}. The embedding model is trained using SGD optimizer with learning rate of 0.05 with momentum 0.9 and weight decay 0.0005 in a similar way to \cite{rfs}. Also, for the training of the embedding model we adopt random data augmentations of crop, color jittering, and random horizontal flip as in \cite{metaridge}. The tensor feature hallucinator is trained in a meta-training regime where $N = 5$ and $K= 20$ for every task. We use Adam optimizer with learning rate of $10^{-5}$ that decays to half at every 10 epochs. We train for 50 epochs where each epoch consists of 600 randomly sampled few-shot learning tasks. At every tasks we generate $M = 50$ class-conditioned samples using our feature tensor hallucinator. At test time we find out that generating more class-conditioned samples improves the accuracy performance therefore we generated $M = 500$ class-conditioned samples.

%\end{document}
 


==> tex/conclusion-1.tex <==
\section{Conclusion}
\label{conclusion}
In this work, we propose a conceptually simple tensor feature hallucinator that improves the state of the art of data augmentation methods in the few-shot learning setting. We provided experimental evidence showing that using a novel loss function and exploiting the structural properties of tensors can provide significant improvement in performance. Notably, the importance of using tensor features is evident through comparison with vector feature hallucinator that is incapable of providing the same improvement in performance. Potential future directions include investigating the performance of our hallucinator in different settings such as in dynamic few-shot learning or incremental learning.


==> tex/exp-1.tex <==
\section{Experiments}
\label{experiments}
%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
%------------------------------------------------------------------------------

\subsection{Competitors}
We compare our method with the rest of the state of the art data augmentation methods for few-shot learning. Most of the data augmentation techniques use ResNet-18 as backbone embedding model, therefore in order to have fair comparisons between methods we also use the same network. %Since only \cite{DTN} provide publicly available official code, we adapted \cite{DTN} to our code to make objective comparisons. Since no official code is available for the rest of the state-of-the-art few-shot classification data-augmentation methods such as: \cite{AFHN, variationalFSL, Ideme, semanticAugmentation, VIFSL} we re-implemented the best data-augmentation method, AFHN \cite{AFHN} and compared it against our method, however this cannot be claimed to be an objective comparison since there might be small details in the code that were ommited from the paper. The methods \cite{AFHN, Ideme, semanticAugmentation} claim that they use the same pre-trained backbone provided from the code of \cite{semanticAugmentation}. It should be noted that \cite{AFHN} uses ReLU activation as the last activation in the encoder, however through our experiments we found it that better results are provided through using the Sigmoid activation function.

\subsection{Setup}

\paragraph{Datasets:}
We carry out experiments on three commonly used few-shot classication benchmark datasets, \emph{mini}Imagenet, CUB and Cifar-FS. Further details regarding each dataset are provided in section \ref{app:datasets}
\paragraph{Tasks:} We consider $N$-way, $K$-shot classification tasks with $N = 5$ randomly sampled novel classes and $K \in \{1, 5\}$ randomly selected examples per class for support set $S$, that is, $L = 5K$ examples in total. For the query set $Q$, we randomly sample $15$ additional examples per class, that is, $M = 75$ examples in total, which is the most common choice in the literature~\cite{tpn, learning2selftrain, transmatch}. \paragraph{Networks:} In order to obtain as fair comparisons as possible with previous data augmentation methods \cite{deltaencoder, semanticAugmentation, Ideme, AFHN}, we use ResNet18 for our embedding model. Our tensor feature hallucinator consists of a conditioner network and generator network. The conditioner network consists of two 2D convolutional layers, with a ReLU activation function in-between, a flattening module to convert the tensors into vectors and a linear layer. The generator network consists of an unflattening module to convert a vector input into a tensor followed by 3 transposed 2D convolutional layers with ReLU activation functions in-between the layers and a sigmoid activation function at the output of the last transposed 2D convolutional layer. In order to compare the performance of using tensor features instead of vector features we adapted our hallucinator accordingly. For the vector feature hallucinator as a conditioner network we use a two-layer fully-connected network  with a ReLU activation in-between the layers. The vector generator uses the same network architecture as the conditioner with an extra sigmoid activation function applied at the output of the last fully-connected layer. Further details regarding implementation details are provided in section \ref{app:implementations}


%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{adjustbox}{width=1\textwidth}
\setlength\tabcolsep{4pt}
\begin{tabular}{lccccccc}
\toprule
\Th{Method}                     & \Th{Backbone} & \mc{2}{\Th{\emph{mini}ImageNet}} & \mc{2}{\Th{CUB}} &  \mc{2}{\Th{cifar-FS}}\\  
                                                &               & 1-shot    & 5-shot & 1-shot    & 5-shot & 1-shot    & 5-shot\\ \midrule
Meta-GAN \cite{metaGAN}                          & ConvNet-4     & 52.71\ci{0.64} & 68.63\ci{0.67}  & - & - & - & -\\
Delta-Encoder$\dagger$ \cite{deltaencoder}                                   & VGG-16        & 59.90\cip     & 69.70\cip & 69.80\ci{0.46} & 82.60\ci{0.35} & 66.70\cip & 79.80\cip\\
SalNet \cite{salnet}                 & ResNet-101    & 62.22\ci{0.87}        & 77.95\ci{0.65} & - & - & - & -\\
DTN \cite{DTN}                                   & Resnet-12     & 63.45\ci{0.86} & 77.91\ci{0.62} & 72.00\cip & 85.10\cip & 71.50\cip & 82.80\cip\\ \midrule

%Baseline\cite{semanticAugmentation}$\dagger$    & ResNet-18     & 52.73          & 73.31 & - & - & - & -\\
Dual TriNet \cite{semanticAugmentation}          & ResNet-18     & 58.80\ci{1.37} & 76.71\ci{0.69} & 69.61\cip & 84.10\cip & 63.41\ci{0.64} & 78.43\ci{0.64}\\ 
IDeMe-Net \cite{Ideme}                           & ResNet-18     & 59.14\ci{0.86} & 74.63\ci{0.74} & - & - & - & -\\ 
AFHN \cite{AFHN}                                 & ResNet-18     & 62.38\ci{0.72} & 78.16\ci{0.56} & 70.53\ci{1.01} & 83.95\ci{0.63} & 68.32\ci{0.93} & 81.45\ci{0.87}\\
VI-Net \cite{VIFSL}                              & ResNet-18     & 61.05\cip & 78.60\cip & 74.76\cip & 86.84\cip & - & -\\ \midrule
Baseline                                     & ResNet-18     & 56.81\ci{0.81}    & 78.31\ci{0.59} & 67.14\ci{0.89} & 86.22\ci{0.50} & 65.71\ci{0.95} & 84.68\ci{0.61}\\
Baseline-KD                                       & ResNet-18     & 59.62\ci{0.85}     & 79.64\ci{0.62} & 70.85\ci{0.90} & 87.64\ci{0.48} & 69.15\ci{0.94} & 85.89\ci{0.59}\\
VF                          & ResNet-18     & 61.92\ci{0.85} & 77.02\ci{0.64}  & 75.25\ci{0.86} & 87.96\ci{0.48} & 72.60\ci{0.93} & 84.26\ci{0.67}\\
\textbf{TF(ours)}                                   & ResNet-18      & \textbf{64.25}\ci{0.85}     & 80.10\ci{0.61} & \textbf{75.83}\ci{0.91} & 88.17\ci{0.48} & 73.88\ci{0.87} & 85.92\ci{0.61}\\
\textbf{TF-ft(ours)}                                   & ResNet-18     & 63.92\ci{0.86}     & \textbf{80.41}\ci{0.60} & 75.39\ci{0.86} & \textbf{88.72}\ci{0.47} & \textbf{73.89}\ci{0.88} & \textbf{87.15}\ci{0.58}\\
%AFHN\cite{AFHN}*                                & ResNet-18     & 54.71     & 70.38 & - & - & - & -\\ 
%AFHN\cite{AFHN}$\_$sgm*                         & ResNet-18     & 58.17     & 72.44 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm*                         & ResNet-18     & 59.76     & 74.38 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm$\_$cr*                   & ResNet-18     & 58.97     & 75.44 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm$\_$cr+sca*               & ResNet-18     & 58.17     & 75.95 & - & - & - & -\\
%VAE$\_$cond                                     & ResNet-18     & 60.79     & 76.94 & - & - & - & -\\
%VAE$\_$cond+sca                                 & ResNet-18     & 59.62     & 76.50 & - & - & - & -\\
%AE$\_$cond$\_$triplet                           & ResNet-18     & 60.30     & 76.42 & - & - & - & -\\
%AE$\_$cond$\_$triplet+sca                       & ResNet-18     & 60.88     & 76.81 & - & - & - & -\\
%VAE$\_$cond$\_$triplet                          & ResNet-18     & 59.75     & 76.08 & - & - & - & -\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{6pt}
\caption{$\dagger$: Delta-encoder uses VGG-16 backbone for \emph{mini}ImageNet and cifar-FS and ResNet-18 backbone for CUB. VF is our feature hallucinator trained with vector features. TF is our tensor feature hallucinator and TF-ft is our tensor feature hallucinator followed by fine-tuning at inference time}
\label{tab:sota}
\end{table*}
%------------------------------------------------------------------------------

==> tex/exp-2.tex <==
\section{Experiments}
\label{experiments}

%------------------------------------------------------------------------------
\newcommand{\ci}[1]{{\tiny $\pm$#1}}
\newcommand{\cip}{\phantom{\ci{0.00}}}
\newcommand{\cim}{\ci{\alert{0.00}}}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------

\subsection{Datasets}

\paragraph{\emph{mini}ImageNet}

This is a widely used few-shot image classification dataset~\cite{matchingNets, ravilstm}. It contains 100 randomly sampled classes from ImageNet~\cite{imagenet}. These 100 classes are split into 64 training (base) classes, 16 validation (novel) classes and 20 test (novel) classes. Each class contains 600 examples (images). We follow the commonly used split provided by~\cite{ravilstm}.

\paragraph{CUB}

This is a fine-grained classification dataset consisting of 200 classes, each corresponding to a bird species. We follow the split defined by~\cite{closerlook, fewshotCUB}, with 100 training, 50 validation and 50 test classes.

\paragraph{CIFAR-FS}

This dataset is derived from CIFAR-100~\cite{cifar100db}, consisting of 100 classes with 600 examples per class. We follow the split provided by~\cite{closerlook}, with 64 training, 16 validation and 20 test classes.

In the experiments using \emph{ResNet-18} as a backbone network all images from all datasets are resized to $224 \times 224$ in a similar way to other data augmentation methods \cite{AFHN, semanticAugmentation, Ideme, VIFSL}. In the experiments using \emph{ResNet-12} as a backbone network all images are resized to $84 \times 84$ in a similar way to \cite{deepEMD}.

%------------------------------------------------------------------------------
\subsection{Setup}
\paragraph{Tasks}

We consider $N$-way, $K$-shot classification tasks with $N = 5$ randomly sampled novel classes and $K \in \{1, 5\}$ examples drawn at random per class as support set $S$, that is, $L = 5K$ examples in total. For the query set $Q$, we draw $15$ additional examples per class, that is, $75$ examples in total, which is the most common choice~\cite{tpn, learning2selftrain, transmatch}. For performance evaluation, we calculate the classification accuracy based on the correctly classified examples from the query set for each task. In order to reduce the variance of our results, for every experiment we sample 600 tasks times  and  report  mean $\%$  of  the accuracy with the 95$\%$ confidence interval in a similar way to \cite{AFHN}.

\paragraph{Competitors}

We compare our method with state-of-the-art data augmentation methods for few-shot learning, including MetaGAN~\cite{metaGAN}, $\Delta$-encoder~\cite{deltaencoder}, salient network (SalNet)~\cite{salnet}, diversity transfer network~(DTN) \cite{DTN}, dual TriNet~\cite{semanticAugmentation}, image deformation meta-network (IDeMe-Net)~\cite{Ideme}, adversarial feature hallucination network (AFHN)~\cite{AFHN} and variational inference network (VI-Net)~\cite{VIFSL}.

%Since only \cite{DTN} provide publicly available official code, we adapted \cite{DTN} to our code to make objective comparisons. Since no official code is available for the rest of the state-of-the-art few-shot classification data-augmentation methods such as: \cite{AFHN, variationalFSL, Ideme, semanticAugmentation, VIFSL} we re-implemented the best data-augmentation method, AFHN \cite{AFHN} and compared it against our method, however this cannot be claimed to be an objective comparison since there might be small details in the code that were ommited from the paper. The methods \cite{AFHN, Ideme, semanticAugmentation} claim that they use the same pre-trained backbone provided from the code of \cite{semanticAugmentation}. It should be noted that \cite{AFHN} uses ReLU activation as the last activation in the encoder, however through our experiments we found it that better results are provided through using the Sigmoid activation function.

\paragraph{Networks}

Many recent competitors \cite{semanticAugmentation, Ideme, AFHN, VIFSL} use ResNet-18 as backbone embedding model. To perform as fair comparison as possible, we carry out experiments using this backbone. Also, we use a pre-trained ResNet-12 as a backbone embeding model from the publicly available code of \cite{deepEMD} to investigate the tranferability and robustness of our tensor hallucinator.

Our \emph{tensor feature hallucinator} (TFH) consists of a conditioner network and a generator network. The \emph{conditioner} $h: \real^{d \times h \times w} \to \real^{d'}$ consists of two convolutional layers with a ReLU activation in-between, followed by flattening and a fully-connected layer. The \emph{generator} used for the ResNet-18 backbone  $g: \real^{k+d'} \to \real^{d \times h \times w}$ consists of concatenation of $z$ and $s_j$ into $(z; s_j) \in \real^{k+d'}$, followed by reshaping to $(k+d') \times 1 \times 1$ and three transpose-convolutional layers with ReLU activation functions in-between and a sigmoid function in the end.  The \emph{generator} used for the ResNet-12 backbone  $g: \real^{k+d'} \to \real^{d \times h \times w}$ consists of concatenation of $z$ and $s_j$ into $(z; s_j) \in \real^{k+d'}$, followed by reshaping to $(k+d') \times 1 \times 1$ and two transpose-convolutional layers with ReLU activation functions in-between and without an activation function in the end. %More details are provided in \autoref{sec:impl}.
The embedding dimension is $d = 512$ and the resolution $h \times w$ is $7 \times 7$ for the ResNet-18 backbone while for the ResNet-12 backbone the embedding dimension is $d = 640$ and the resolution $h \times w$ is $5 \times 5$.

The convolutional layers of the \emph{conditioner} use kernels of size $3 \times 3$ and stride 1 and in the input layer we also use padding 1 for both backbones. The dimension of the \emph{class-conditional vector} is set to $d' = 1024$. All transpose-convolutional layers of the \emph{generator} use kernels of size $3 \times 3$, stride 1 and 512 channels for the ResNet-18 backbone features and 640 channels for the ResNet-12 backbone features. The dimension of $z \sim \normal(\vzero,I_{k})$ is $k = 1024$. %The tensor dimensions of all conditioner layers for ResNet-18 backbone features are $[512 \times 7 \times 7]$, $[256 \times 5 \times 5]$, $[6400]$ (flattening) and $[1024]$. The tensor dimensions of all conditioner layers for ResNet-12 backbone features are $[640 \times 5 \times 5]$, $[320 \times 3 \times 3]$, $[2880]$ (flattening) and $[1024]$. %The tensor dimensions of all generator layers for ResNet-18 backbone features are $[2048 \times 1 \times 1]$, $[512 \times 3 \times 3]$, $[512 \times 5 \times 5]$, and $[512 \times 7 \times 7]$. The tensor dimensions of all generator layers for ResNet-18 backbone features are $[2048 \times 1 \times 1]$, $[640 \times 3 \times 3]$, and $[640 \times 5 \times 5]$.

\subsection{Training}

For the \emph{embedding model}, similarly to \cite{rfs}, we use SGD optimizer with learning rate 0.05, momentum 0.9 and weight decay 0.0005. For data augmentation, as in \cite{metaridge}, we adopt random crop, color jittering, and horizontal flip.

The \emph{tensor feature hallucinator} is trained in a meta-training regime with $N = 5$ classes, $K = 20$ examples per class and  generation of $M = 50$ class-conditioned examples in every task. We use Adam optimizer with initial learning rate $10^{-5}$, decaying by half at every 10 epochs. We train for 50 epochs, where each epoch consists of 600 randomly sampled few-shot learning tasks. At test time, we generate class-conditioned examples and augment the support set. We also provide an improved solution, called TFH-ft, where our tensor feature hallucinator is \emph{fine-tuned} on novel-class support examples at inference. We noticed that the ideal number of generated class-conditioned tensor features varies with respect to the available support examples per class, backbone architecture and whether the TFH is fine-tuned. In the ResNet-18 experiments  we generated $M = 100$ and $M=2$ per class in the 1-shot and 5-shot setting respectively using TFH and $M=100$ using TFH-ft. In the ResNet-12 experiments we generated $M = 1$ and $M = 2$ per class in 1-shot and 5-shot settings for standard TFH and TFH-ft respectively. Further analysis regarding the effect on the number of generated tensor features is provided in section \ref{sec:generated_features}.

Our TFH-ft version uses the novel-class support examples to fine-tune all of its parameters. In the fine-tuning stage, we use exactly the same loss function as in the hallucinator training phase~\eq{mse} and we fine-tune for $k$ steps using Adam optimizer and learning rate of $\gamma$. The values of $k$ and $\gamma$ where calculated on miniImagenet for both ResNet-18 and ResNet-12 using the valitation dataset and were used accordingly in all test experiments on all datasets. Table \ref{tab:hyperparameters} provides the values $k$ and $\gamma$ used for each backbone.

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
%\begin{adjustbox}{width=1\linewidth}
\setlength\tabcolsep{4pt}
\begin{tabular}{lcccccc} \toprule
\Th{Backbone}                   & \mc{2}{\Th{1-shot}} & \mc{2}{\Th{5-shot}}\\
                        & $k$             & $\gamma$   &$k$             & $\gamma$    \\ \midrule
ResNet-18               & 15     & $10^{-7}$ & 10& $10^{-4}$ \\
ResNet-12          & 2     & $10^{-4}$ & 5&  $10^{-7}$ \\ %& 67.76\ci{0.85}     & 84.88\ci{0.55}\\
\bottomrule
\end{tabular}
%\end{adjustbox}
\vspace{6pt}
\caption{Hyperparameters used in TFH-ft experiments for all datasets.}
\label{tab:hyperparameters}
\end{table}
%------------------------------------------------------------------------------




%------------------------------------------------------------------------------
\begin{table*}
\small
\centering
\begin{adjustbox}{width=1\textwidth}
\setlength\tabcolsep{4pt}
\begin{tabular}{lccccccc} \toprule
\Th{Method}                                      & \Th{Backbone} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{CUB}}                          & \mc{2}{\Th{CIFAR-FS}}                     \\
                                                 &               & 1-shot              & 5-shot              & 1-shot              & 5-shot              & 1-shot              & 5-shot              \\ \midrule
MetaGAN \cite{metaGAN}                           & ConvNet-4     & 52.71\ci{0.64}      & 68.63\ci{0.67}      & --                  & --                  & --                  & --                  \\
$\Delta$-Encoder$\dagger$ \cite{deltaencoder}    & VGG-16        & 59.90\cip           & 69.70\cip           & 69.80\ci{0.46}      & 82.60\ci{0.35}      & 66.70\cip           & 79.80\cip           \\
SalNet \cite{salnet}                             & ResNet-101    & 62.22\ci{0.87}      & 77.95\ci{0.65}      & --                  & --                  & --                  & --                  \\
DTN \cite{DTN}                                   & Resnet-12     & 63.45\ci{0.86}      & 77.91\ci{0.62}      & 72.00\cip           & 85.10\cip           & 71.50\cip           & 82.80\cip           \\ \midrule
%Baseline\cite{semanticAugmentation}$\dagger$    & ResNet-18     & 52.73               & 73.31               & --                  & --                  & --                  & --                  \\
Dual TriNet \cite{semanticAugmentation}          & ResNet-18     & 58.80\ci{1.37}      & 76.71\ci{0.69}      & 69.61\cip           & 84.10\cip           & 63.41\ci{0.64}      & 78.43\ci{0.64}      \\
IDeMe-Net \cite{Ideme}                           & ResNet-18     & 59.14\ci{0.86}      & 74.63\ci{0.74}      & --                  & --                  & --                  & --                  \\
AFHN \cite{AFHN}                                 & ResNet-18     & 62.38\ci{0.72}      & 78.16\ci{0.56}      & 70.53\ci{1.01}      & 83.95\ci{0.63}      & 68.32\ci{0.93}      & 81.45\ci{0.87}      \\
VI-Net \cite{VIFSL}                              & ResNet-18     & 61.05\cip           & 78.60\cip           & 74.76\cip           & 86.84\cip           & --                  & --                  \\ \midrule
Baseline~\eq{cls}                                & ResNet-18     & 56.81\ci{0.81}      & 78.31\ci{0.59}      & 67.14\ci{0.89}      & 86.22\ci{0.50}      & 65.71\ci{0.95}      & 84.68\ci{0.61}      \\
Baseline-KD~\eq{kl}                              & ResNet-18     & 59.62\ci{0.85}      & 79.31\ci{0.62}      & 70.85\ci{0.90}      & 87.64\ci{0.48}      & 69.15\ci{0.94}      & 85.89\ci{0.59}      \\
VFH (ours)                                       & ResNet-18     & 61.88\ci{0.85}      & 79.63\ci{0.61}      & 75.44\ci{0.85}      & 87.82\ci{0.47}      & 72.31\ci{0.91}      & 85.64\ci{0.64}      \\
\tb{TFH (ours)}                                  & ResNet-18     & 64.49\ci{0.84} & 79.94\ci{0.60}       & 75.66\ci{0.85} & 88.39\ci{0.49}      & 73.77\ci{0.85}      & 86.68\ci{0.63}      \\
\tb{TFH-ft (ours)}                               & ResNet-18     & \tb{65.07}\ci{0.82}      & \tb{80.81}\ci{0.61} & \tb{75.76}\ci{0.83}  & \tb{88.60}\ci{0.47} & \tb{74.77}\ci{0.90} & \tb{86.88}\ci{0.59}\\
%AFHN\cite{AFHN}*                                & ResNet-18     & 54.71     & 70.38 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm*                         & ResNet-18     & 58.17     & 72.44 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm*                         & ResNet-18     & 59.76     & 74.38 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm$\_$cr*                   & ResNet-18     & 58.97     & 75.44 & - & - & - & -\\
%AFHN\cite{AFHN}$\_$sgm$\_$cr+sca*               & ResNet-18     & 58.17     & 75.95 & - & - & - & -\\
%VAE$\_$cond                                     & ResNet-18     & 60.79     & 76.94 & - & - & - & -\\
%VAE$\_$cond+sca                                 & ResNet-18     & 59.62     & 76.50 & - & - & - & -\\
%AE$\_$cond$\_$triplet                           & ResNet-18     & 60.30     & 76.42 & - & - & - & -\\
%AE$\_$cond$\_$triplet+sca                       & ResNet-18     & 60.88     & 76.81 & - & - & - & -\\
%VAE$\_$cond$\_$triplet                          & ResNet-18     & 59.75     & 76.08 & - & - & - & -\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{6pt}
\caption{Comparison of our proposed method variants and baselines to state of the art on few-shot classification datasets. $\dagger$: Delta-encoder uses VGG-16 backbone for \emph{mini}ImageNet and CIFAR-FS and ResNet-18 for CUB. Baseline~\eq{cls}, Baseline-KD~\eq{kl}: prototypical classifier at inference, no feature generation. VFH: our vector feature hallucinator; TFH: our tensor feature hallucinator; TFH-ft: our tensor feature hallucinator followed by fine-tuning at inference.}
\label{tab:sota}
\end{table*}
%------------------------------------------------------------------------------



% %------------------------------------------------------------------------------
% \begin{table}
% \small
% \centering
% \begin{adjustbox}{width=1\linewidth}
% \setlength\tabcolsep{4pt}
% \begin{tabular}{lccccccc} \toprule
% \Th{Method}                                      & \Th{Backbone} & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{CUB}}\\
%                                                  &               & 1-shot              & 5-shot              & 1-shot              & 5-shot \\ \midrule
%                                                  \mc{6}{\Th{Logistic regression classifier}}\\ \midrule
% Baseline~\eq{cls}                                & ResNet-18     & 59.20\ci{0.82}      & 77.71\ci{0.61}      & 69.44\ci{0.86}      & 86.19\ci{0.49} \\
% Baseline-KD~\eq{kl}                              & ResNet-18     & 61.83\ci{0.82}      & 79.27\ci{0.61}      & 72.74\ci{0.88}      & 87.71\ci{0.49}  \\
% VFH (ours)                                       & ResNet-18     & 61.41\ci{0.83}      & 78.54\ci{0.62}      & 74.43\ci{0.86}      & 87.90\ci{0.50}  \\
% \tb{TFH (ours)}                                  & ResNet-18     & \tb{63.94}\ci{0.88} & 79.16\ci{0.63}      & \tb{75.05}\ci{0.93} & 88.22\ci{0.49}   \\
% \tb{TFH-ft (ours)}                               & ResNet-18     & -      & \tb{79.76}\ci{0.60} & -      & -\\ \midrule
%                                                  \mc{6}{\Th{Support vector machines classifier}}\\ \midrule
% Baseline~\eq{cls}                                & ResNet-18     & 57.12\ci{0.84}      & 76.45\ci{0.62}      & 67.24\ci{0.87}      & 84.72\ci{0.52} \\
% Baseline-KD~\eq{kl}                              & ResNet-18     & 60.21\ci{0.84}      & 78.28\ci{0.61}      & 71.23\ci{0.89}      & 86.34\ci{0.52}  \\
% VFH (ours)                                       & ResNet-18     & 59.42\ci{0.83}      & 77.71\ci{0.64}      & 71.89\ci{0.888}      & 86.63\ci{0.49}  \\
% \tb{TFH (ours)}                                  & ResNet-18     & \tb{64.23}\ci{0.88} & 79.49\ci{0.60}      & \tb{75.75}\ci{0.90} & 88.26\ci{0.47}   \\
% \tb{TFH-ft (ours)}                               & ResNet-18     & 63.82\ci{0.85}      & \tb{79.96}\ci{0.58} & 74.54\ci{0.91}      & \tb{88.33}\ci{0.48}\\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \vspace{6pt}
% \caption{Comparison of our proposed method variants and baselines using different losses}
% \label{tab:dif_losses}
% \end{table}
% %------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{adjustbox}{width=1\linewidth}
\setlength\tabcolsep{4pt}
\begin{tabular}{lcccccc} \toprule
\Th{Method}                                     & \mc{2}{\Th{\emph{mini}ImageNet}}          & \mc{2}{\Th{CUB}}\\
                                                & 1-shot              & 5-shot              & 1-shot    & 5-shot \\ \midrule
                                                 \mc{5}{\Th{Logistic regression classifier}}\\ \midrule
Baseline~\eq{cls}                               & 59.20\ci{0.82}      & 77.71\ci{0.61}      & 69.44\ci{0.86}      & 86.19\ci{0.49} \\
Baseline-KD~\eq{kl}                             & 61.83\ci{0.82}      & 79.27\ci{0.61}      & 72.74\ci{0.88}      & 87.71\ci{0.49}  \\
VFH (ours)                                      & 62.37\ci{0.83}      & 79.70\ci{0.59}      & 75.06\ci{0.88}      & 87.95\ci{0.46}  \\
\tb{TFH (ours)}                                 & 64.03\ci{0.84} & 79.93\ci{0.60}      & 75.08\ci{0.85} & \tb{88.82}\ci{0.46}   \\
\tb{TFH-ft (ours)}                              & \tb{64.83}\ci{0.82}      & \tb{80.49}\ci{0.61} & \tb{75.43}\ci{0.85}      & 88.52\ci{0.48}\\ \midrule
                                                 \mc{5}{\Th{Support vector machines classifier}}\\ \midrule
Baseline~\eq{cls}                               & 57.12\ci{0.84}      & 76.45\ci{0.62}      & 67.24\ci{0.87}      & 84.72\ci{0.52} \\
Baseline-KD~\eq{kl}                             & 60.21\ci{0.84}      & 78.28\ci{0.61}      & 71.23\ci{0.89}      & 86.34\ci{0.52}  \\
VFH (ours)                                      & 61.95\ci{0.85}      & 79.15\ci{0.60}      & 75.43\ci{0.85}      & 87.46\ci{0.47}  \\
\tb{TFH (ours)}                                 & 64.20\ci{0.83} & 79.62\ci{0.60}      & 75.64\ci{0.85} & \tb{88.74}\ci{0.45}   \\
\tb{TFH-ft (ours)}                              & \tb{65.06}\ci{0.82}     & \tb{80.33}\ci{0.60} & \tb{75.77}\ci{0.83}      & 88.22\ci{0.46}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{6pt}
\caption{Comparison of our proposed method variants and baselines using different losses. ResNet-18 is used as the backbone in this experiment.}
\label{tab:dif_losses}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
%\begin{adjustbox}{width=1\linewidth}
\setlength\tabcolsep{4pt}
\begin{tabular}{lcccc} \toprule
\Th{Method}                                       & \mc{2}{\Th{\emph{mini}ImageNet}}\\ %& \mc{2}{\Th{CUB}}\\ \\
                        & 1-shot              & 5-shot      \\%& 1-shot              & 5-shot\\ \midrule
                        \mc{3}{\Th{Prototypical classifier}}\\ \midrule
Baseline                & 59.94\ci{0.84}     &78.65\ci{0.61}  \\        %& 66.72\ci{0.90}     & 84.27\ci{0.59}\\
\tb{TFH (ours)}         & 64.28\ci{0.84}    & 79.72\ci{0.59} \\ %& 67.76\ci{0.85}     & 84.88\ci{0.55}\\
\tb{TFH-ft (ours)}      & \tb{65.22}\ci{0.83}      & \tb{79.86}\ci{0.62}\\ \midrule         %& \tb{68.23}\ci{0.86}     & \tb{85.20}\ci{0.56}\\ \midrule
            \mc{3}{\Th{Logistic regression classifier}}\\ \midrule
Baseline                & 61.83\ci{0.85}      &79.60\ci{0.60} \\%& 68.49\ci{0.49}     & 84.75\ci{0.59}\\
\tb{TFH (ours)}         & 65.07\ci{0.84} & 80.21\ci{0.58}\\%& 68.05\ci{0.89}     & 85.13\ci{0.54}\\
\tb{TFH-ft (ours)}      &  \tb{65.60}\ci{0.82}   & \tb{80.53}\ci{0.57}\\%& \tb{68.83}\ci{0.87}     & \tb{85.42}\ci{0.56}\\
\midrule
\mc{3}{\Th{Support vector machines classifier}}\\ \midrule
Baseline              & 59.94\ci{0.84}      & 78.43\ci{0.60} \\%& 66.72\ci{0.90}     & 83.29\ci{0.60}\\
\tb{TFH(ours)}       & 59.94\ci{0.86} & 78.48\ci{0.60}\\%& 68.03\ci{0.85}     & \tb{84.21}\ci{0.56}\\
%\tb{TFH(ours)-100}       & 60.16\ci{0.88} & 78.08\ci{0.63}\\%& 68.03\ci{0.85}     & \tb{84.21}\ci{0.56}\\
\tb{TFH-ft(ours)}      &  \tb{60.25}\ci{0.85}   & \tb{78.98}\ci{0.59} \\%& \tb{68.26}\ci{0.86}     & 84.07\ci{0.56}\\ %\midrule
\bottomrule
\end{tabular}
%\end{adjustbox}
\vspace{6pt}
\caption{Comparison of our proposed method using the publicly available pre-trained ResNet-12 backbone provided by \cite{deepEMD}. For the prototypical and logistic regression classifiers we generate 2 class conditional tensor features per class,}
\label{tab:comb_res12}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
% \begin{table}
% \small
% \centering
% \begin{adjustbox}{width=1\linewidth}
% \setlength\tabcolsep{4pt}
% \begin{tabular}{lcccccc} \toprule
% \Th{Method}                                       & \mc{2}{\Th{\emph{mini}ImageNet}} & \mc{2}{\Th{CUB}}\\ \\
%                         & 1-shot              & 5-shot      & 1-shot              & 5-shot\\ \midrule
%                         \mc{5}{\Th{Prototypical classifier}}\\ \midrule
% DeepEMD                & 64.68\ci{0.82}     &81.73\ci{0.57}  & 75.26\ci{0.83}   & 88.61\ci{0.52}\\
% \tb{DeepEMD + TFH (ours)}         &-    & -    & -    & -\\
% \tb{DeepEMD + TFH-ft (ours)}      & -     & -         & -     &-\\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \vspace{6pt}
% \caption{Combination of tensor hallucination and deepEMD using the publicly available pre-trained ResNet-12 backbone provided by \cite{deepEMD}.}
% \label{tab:comb_other_methods}
% \end{table}

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{adjustbox}{width=1\linewidth}
\setlength\tabcolsep{4pt}
\begin{tabular}{lcccccc} \toprule
\Th{Gen. Samples}              & \mc{2}{\Th{ResNet-18}} & \mc{2}{\Th{ResNet-12}}\\ \\
                        & 1-shot              & 5-shot      & 1-shot              & 5-shot\\ \midrule
                        \mc{5}{\Th{Prototypical classifier}}\\ \midrule
0   & 59.62\ci{0.85}      & 79.31\ci{0.62} & 59.94\ci{0.84}     & 78.65\ci{0.61} \\
1   & 62.43\ci{0.83}     &79.33\ci{0.62}          & \tb{64.28}\ci{0.84}    & \tb{79.72}\ci{0.59}\\
2   & 63.57\ci{0.87}     &\tb{79.94}\ci{0.60}          & 64.16\ci{0.79}    & 79.50\ci{0.60}\\
5   & 64.42\ci{0.83}     & 79.77\ci{0.61}    & 63.84\ci{0.85}     & 78.85\ci{0.63}\\
10  & 63.90\ci{0.81}    & 79.64\ci{0.60}     & 63.57\ci{0.82} & 77.94\ci{0.67}\\
50  & 63.44\ci{0.86}    &79.43\ci{0.63}         & 63.03\ci{0.83}    & 75.46\ci{0.73}\\
100 & \tb{64.49}\ci{0.84}    & 79.27\ci{0.60}    &  62.83\ci{0.82} & 74.99\ci{0.73}\\
500 & 64.25\ci{0.85} & 79.71\ci{0.62}        & 63.38\ci{0.85}     & 74.50\ci{0.73}\\
1000& 63.76\ci{0.87}     & 79.52\ci{0.62}         & 63.47\ci{0.79} & 74.33\ci{0.72}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{6pt}
\caption{Comparison of our proposed method, TFH without fine-tuning, on \emph{mini}ImageNet with different number of generated samples}
\label{tab:gen_samples}
\end{table}
%------------------------------------------------------------------------------

%------------------------------------------------------------------------------
\begin{table}
\small
\centering
\begin{adjustbox}{width=1\linewidth}
\setlength\tabcolsep{4pt}
\begin{tabular}{lcccccc} \toprule
\Th{Method}              & \mc{2}{\Th{\emph{mini}Imagenet}\textrightarrow \Th{CUB}} & \mc{2}{\Th{\emph{mini}Imagenet}\textrightarrow\Th{CIFAR-FS}}\\ \\
                        & 1-shot              & 5-shot      & 1-shot              & 5-shot\\ \midrule
                        \mc{5}{\Th{Prototypical classifier}}\\ \midrule
Baseline~\eq{cls}               & 43.14\ci{0.78}     & 62.20\ci{0.70}         & 50.25\ci{0.86}     & 69.43\ci{0.74}\\
Baseline-KD~\eq{kl}               & 44.40\ci{0.82}     & \tb{63.83}\ci{0.73}         & 51.54\ci{0.89}     & 70.40\ci{0.72}\\
\tb{VFH (ours)}         & 44.77\ci{0.79}     & 62.61\ci{0.73}   & 50.36\ci{0.87}    & 69.31\ci{0.74}\\
\tb{TFH (ours)}         & 45.67\ci{0.80}     & 63.08\ci{0.73}   & 51.82\ci{0.89}    & 69.77\ci{0.76}\\
\tb{TFH-ft (ours)}      & \tb{45.96}\ci{0.80}     & 63.64\ci{0.74}        &  \tb{53.07}\ci{0.86}    & \tb{71.29}\ci{0.75}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{6pt}
\caption{Few-shot cross-domain experiments using ResNet-18 as backbone. The backbone is trained on \emph{mini}Imagenet}
\label{tab:cross_domain}
\end{table}
%------------------------------------------------------------------------------
\paragraph{Baselines}

To validate the benefit of generating tensor features, we also implement a \emph{vector feature hallucinator} (VFH), where we use $\bar{f}_{\theta'}: \cX \to \real^d$ including GAP~\eq{kl} as embedding model. In this case, the \emph{conditioner} $h: \real^d \to \real^{d'}$ consists of two fully-connected layers with a ReLU activation in-between. The \emph{generator} $g: \real^{k+d'} \to \real^d$ also consists of two fully-connected layers with a ReLU activation in-between and a sigmoid function in the end. In our \emph{vector feature hallucinator} (VFH), the dimensions of the \emph{class-conditional vector} as well as the hidden layers of both the \emph{conditioner} and the \emph{generator} are all set to 512.

Finally, we experiment with baselines consisting of the embedding network $f_\theta$~\eq{cls} or $f_{\theta'}$~\eq{kl} at representation learning and a prototypical classifier at inference, without feature hallucination. We refer to them as Baseline~\eq{cls} and Baseline-KD~\eq{kl} respectively.



\subsection{Comparison with state of the art data augmentation methods}

\autoref{tab:sota} compares our method with the state of the art. Most important are comparisons with \cite{semanticAugmentation, Ideme, AFHN, VIFSL}, which use the same backbone, ResNet-18. Our tensor feature hallucinator provides new state of the art performance in all datasets in both 1-shot and 5-shot settings, outperforming all competing few-shot data augmentation methods. \emph{Fine-tuning} at inference is mostly beneficial, impressively even in the 1-shot setting fine-tuning can provide benefit which shows that our tensor hallucinator is robust and avoids overfitting. Also, it is clear that the \emph{tensor feature hallucinator} is superior to the vector feature hallucinator highlighting the importance of using tensor features, while the latter is still very competitive highlighting the effectiveness of our proposed loss function. \emph{Self-distillation} also provides a significant improvement in performance in all experiments.


\subsection{Experiments with different classifiers}
\label{sec:dif_cls}
In order to investigate the robustness of our tensor hallucinator we investigate its performance using different classifiers instead of the prototypical classifier \cite{prototypical} such as logistic regression and support vector machines classifiers. Both logistic regression and support vector machines classifiers are implemented using the scikit-learn framework \cite{sklearn}. It can be clearly seen that our tensor hallucinator still provides the best accuracy results irrespective of the classifier used thus highlighting its robustness and potential to be used in different classification methods.

\subsection{Experiments with ResNet-12}
In order to investigate the transferability of our method we carried out experiments using a different backbone network, the widely used \emph{ResNet-12}. We used the publicly available pre-trained networks provided by deepEMD \cite{deepEMD}\footnote{\url{https://github.com/icoz69/DeepEMD}}. We compared the baseline model without using our tensor feature hallucinator denoted as Baseline. We carried experiments in the \emph{mini}Imagenet dataset comparing the baseline with and without the use of our tensor feature hallucinator using three different classifiers, prototypical, logistic regression and support vector machines classifier. Our tensor hallucinator provides the best results in all settings with a significant performance gain of $\sim$ 5\% in 1-shot learning in prototypical and logistic regression classifiers.

\subsection{Effect of number of generated samples}
\label{sec:generated_features}
We investigated the effect of the number of generated samples used in the classification performance using both backbones ResNet-18 and ResNet-12 which can be seen from \ref{tab:gen_samples}. Interestingly we observe that for both backbones, using only 1 or 2 generated samples per class provides a significant performance improvement of around 4\% in the 1-shot setting when compared to 0 generated samples. Interestingly, for the ResNet-18 bacbkone the performance does not seem to degrade significantly in both 1-shot and 5-shot settings even when 1000 samples per class are generated, outperforming the respective baseline and highlighting the efficacy of our hallucinator. In the ResNet-12 backbone it can be observed that in the 1-shot setting any number of generated samples also improves significantly the performance. However this is not the case in the 5-shot setting and it can be observed that as the number of generated samples increases the performance degrades which can possibly be attributed to the fact that no sigmoid function is used in the output of the hallucinator for the ResNet-12 experiments thus the generated features can be much more scattered. Nevertheless it is clear that with the appropriate number of generated samples our hallucinator provides significance performance improvement with both backbones.%Also in the ResNet-12 experiment, it can be observed that the performance improves significantly with more samples. However this is not the case in the ResNet-18 experiment where the performance does not seem to have either a positive or negative effect with more samples. This can be attributed to the fact that even with 2 samples there is a great increase in performance and there is no room for further increase with more samples.

\subsection{Cross-domain few-shot}
We investigated the ability of our tensor hallucinator to address domain shift carrying out experiments in the cross-domain few-shot classification setting as proposed by \cite{closerlook}. We used our pre-trained ResNet-18 backbone and our tensor hallucinator trained on the \emph{miniImagenet} $D_{\base}$ dataset and evaluated the performance on $D_{\novel}$ of both CUB and CIFAR-FS dataset. It can be seen from Table \ref{tab:cross_domain} that our tensor hallucinator can address the domain shift effectively especially in the 1-shot setting even without any fine-tuning. Even though the results are less impressive in the 5-shot setting, still our hallucinator shows positive results outperforming the Baseline-KD in the \emph{mini}Imagenet \textrightarrow CIFAR-FS while being almost on par in performance in \emph{mini}Imagenet \textrightarrow CUB.


%------------------------------------------------------------------------------
\begin{figure}[h]
\centering
\includegraphics[width=0.8\linewidth, height=0.22\textheight]{imgs/tsne_border.png}
\caption{t-SNE visualization of the augmented support set features in 1-shot \emph{mini}Imagenet setting using ResNet-18 backbone. Different classes are indicated by different colours.}
\label{fig:idea}
\end{figure}
%------------------------------------------------------------------------------
\subsection{Feature embeddings}
In order to visualize the generative ability of our tensor feature hallucinator we utilize the t-SNE visualization tool \cite{tsne}. At inference stage, we sample a random 5-way, 1-shot episode and use the support set to generate 500 novel embedding from each sampled class and augment the support set. We apply t-SNE on the augmented support set and visualize the features in a two-dimensional map. Impressively it can be clearly seen that all feature from each class are clustered together with very distinct boundaries meaning that our hallucinator can identify the underlying distribution of each class generating class conditional samples that can be used for training a classifier successfully.



==> tex/intro-1.tex <==
\section{Introduction}
\label{intro}
Deep learning continuously keeps improving the state of the art performance in multiple different areas such as computer vision \cite{imagenet} and natural language understanding \cite{language}. However, even though the success of deep learning models is undeniable, a fundamental limitation of them is their dependence on large amounts of labeled data. This limitation inhibits the applicability of the state of the art deep learning techniques in real-world problems where the cost of annotating data is high and data can be scarce, i.e. rare species classification.

In order to address this limitation, the field of few-shot learning has attracted significant research interest in recent years. Multiple different lines of research have been proposed over the years to address the few-shot learning problem. One of the most common lines of research is meta-learning, addressing the problem of few-shot learning by leveraging training episodes that mimic a few-shot task by having small number of classes and limited number of samples per class. Meta-learning approaches can further be partitioned in optimization-based approaches that attempt to learn to update the learner's meta-parameters \cite{MAML, CAVIA, reptile, ravilstm}, metric-based approaches that attempt to learn a discriminative embedding space where samples from a novel task are easy to classify \cite{siamese, prototypical, relationnet, matchingNets} and model-based approaches that depend on specific model architectures to learn how to update the learner's parameters effectively \cite{santoro, metaNet}.

Beyond meta-learning methods, other approaches include methods that leverage the manifold structure of the data either by label propagation, embedding propagation or through the use of graph neural networks \cite{fewshotGNN1, fewshotGNN2, tpn, ilpc} and domain adaptation techniques that attempt to reduce the domain shifts between source and target domains \cite{domain_one, l2cluster}. Another line of research constitutes of data augmentation methods that attempt to tackle the data deficiency by augmenting the few-shot training dataset with extra samples \cite{AFHN, VIFSL, semanticAugmentation, Ideme, antoniou, metaGAN}.

Our work falls into the data augmentation category. We show that using a simple loss function to train a feature hallucinator can provide significant performance boost and outperform the current state of the art methods that use more complex and sophisticated methods such as: wGANS, VAEs and networks trained to transfer sample diversity. Also, to the best of our knowledge, we are the first to propose to generate tensor features instead of vector features in the few-shot setting.%These methods in general attempt to either train a generator or identify a way to augment the few-shot dataset during inference in time such that the classification performance is improved. However most of the proposed data augmentation techniques use sophisticated generators borrowed from the general deep learning literature. For example \cite{AFHN} trains a wGAN based feature hallucinator combined with two regularizer while \cite{VIFSL} trains a VAE model where the few labelled examples are used to infer the mean and variance of each class. \cite{DTN} to  transfer  latent  diversities  in order to combine them with support features to generate new features, \cite{Ideme} train a deformation network to fuse reference images with novel images. However, most of these methods follow sophisticated training regimes, such as training a wGAN, VAE, sampling reference images in order to train a generator successfully. In contrast in our work we simply show that using a very simple loss function is more than enough to train a feature hallucinator showing at the same time that there is no added benefit from using any complex training regime.

%Our contributions are summarized below:
%\begin{itemize}
%    \item We show that using a very simple loss function to train a feature hallucinator provides similar performance to sophisticated training regimes such as wGANs and VAEs.
%    \item To the best of our knowledge, we are the first to  propose to generate feature tensors instead of vector features in the few-shot setting, thus exploiting the spatial and structural properties of the feature tensors.
%    \item We achieve new state of the art results comparing all \emph{few-shot} data augmentation techniques.
%    \item We show that our method can be combined with other methods successfully
%\end{itemize}

==> tex/intro-2.tex <==
\section{Introduction}
\label{intro}
Deep learning continuously keeps improving the state of the art in multiple different fields, such as natural language understanding~\cite{language} and computer vision~\cite{imagenet}. However, even though the success of deep learning models is undeniable, a fundamental limitation is their dependence on large amounts of labeled data. This limitation inhibits the application of state of the art deep learning methods to real-world problems, where the cost of annotating data is high and data can be scarce, \eg, as in the problem of rare species classification.


To address this limitation, \emph{few-shot learning} has attracted significant interest in recent years with multiple different approaches  proposed over the years to address this problem.
One of the most widely researched approaches is \emph{meta-learning},
% addressing the problem of few-shot learning by leveraging training episodes that
where training episodes
mimic a few-shot task by having a small number of classes and a limited number of examples per class. Meta-learning approaches can further be partitioned in \emph{optimization-based}~\cite{MAML, CAVIA, reptile, ravilstm}, \emph{metric-based}~\cite{siamese, prototypical, relationnet, matchingNets} and \emph{model-based}~\cite{santoro, metaNet}. %Meta-learning approaches can further be partitioned in \emph{optimization-based}, learning to update the learner's meta-parameters~\cite{MAML, CAVIA, reptile, ravilstm}, \emph{metric-based}, learning a discriminative embedding space where novel examples are easy to classify~\cite{siamese, prototypical, relationnet, matchingNets} and \emph{model-based}, depending on specific model architectures to learn how to update the learner's parameters effectively~\cite{santoro, metaNet}.


%------------------------------------------------------------------------------
\begin{figure*}[ht]
\centering
%\includegraphics[width=\linewidth, height=0.30\textheight]{fig/idea_shape.png}
\includegraphics[width=\textwidth, height=0.18\textheight]{fig/idea_1line_improved.png}
\caption{Overview of our method. 1) Map the support and query set into tensor features through the pre-trained backbone network. 2) Calculate the tensor prototype of each class. 3) Calculate the class conditional vectors of each class through the conditioner network. Sample $M$ samples from a Normal distribution. 5) Generate class-conditional tensor features. 6) Augment the support tensors with the generated tensors. 7) Perform global average pooling to all support and query tensors, re-calculate the class prototypes and classify each query vector.}
\label{fig:overview}
\end{figure*}
%------------------------------------------------------------------------------

Beyond meta-learning, other approaches include leveraging the \emph{manifold structure} of the data, by label propagation, embedding propagation or graph neural networks~\cite{fewshotGNN1, fewshotGNN2, tpn, ilpc}. \emph{Domain adaptation} methods that aim at reducing the domain shift between source and target domains~\cite{domain_one, l2cluster}. \emph{Data augmentation} methods, that address data deficiency by augmenting the few-shot training dataset with extra examples in the image space~\cite{Ideme, metaGAN} and in the feature space~\cite{semanticAugmentation, AFHN, VIFSL}. The most recent methods in this line of research go beyond standard augmentation~\cite{imagenet} towards \emph{synthetic data generation} and \emph{hallucination}, achieving a greater extent of diversity by adapting the state of the art techniques in \emph{synthetic data generation} in the few-shot learning setting. %\iavr{Check this again, remove color and comment when done.}
% \cite{AFHN, VIFSL, semanticAugmentation, Ideme, antoniou, metaGAN}.

However, the vast majority of \emph{synthetic data generation} research focuses on generating high-quality, high-resolution images assuming access to a large amount of available data. %It is unclear how these techniques can be adapted successfully in situations where the available data is limited.
Also, the main metrics used to compare generative models are Fréchet Inception Distance (FID)~\cite{FID} and Inception score (IS) ~\cite{IS} which focus in calculating whether the generated data is  realistic. Generating high quality, realistic data does not necessarily mean improvement in the performance of "downstream tasks" such as classification. Due to the aforementioned reasons it unclear whether and how the current state of the art generative models can be used successfully in the \emph{few-shot learning} setting.

Our work falls in the category of \emph{synthetic data generation} for few-shot learning. We explore the potential of using a simple generative model to improve the classification performance in the few-shot learning setting by leveraging tensors instead of vector features. Through our experimental results it is evident that our proposed generative model can provide state of the art results and outperforms much more sophisticated generative models. An overview of our proposed method can be seen in Figure \ref{fig:overview}. Our contributions are summarized below:
\begin{itemize}
    \item We propose a novel loss function to train a feature hallucinator that is much simpler than the current state of the art few-shot synthetic data generation methods.% outperforming the current state of the art few-shot synthetic data generation methods using more complex and sophisticated generation methods, such as wGAN~\cite{AFHN}, VAE~\cite{VIFSL} and networks trained to transfer example diversity~\cite{DTN}.

    \item We are the first to propose generating \emph{tensor features} instead of vector features in the few-shot setting, leveraging the structural properties of tensors in the process.

    \item We carry out experiments on three commonly used few-shot classication benchmark datasets: \emph{mini}Imagenet, CUB and CIFAR-FS comparing to other related methods setting a new state of the art.% the superiority of our approach.

    \item We demonstrate the robustness of our tensor feature hallucinator through a wide range of few-shot experiments, such as using different backbone networks, different classifiers and in the challenging setting of cross-domain few-shot learning.
\end{itemize}

%Our work falls into the category of data augmentation in the feature space. We show that using a simple loss function to train a feature hallucinator can outperform other state of the art few-shot data augmentation methods that use more complex and sophisticated generation methods, such as wGAN~\cite{AFHN}, VAE~\cite{VIFSL} and networks trained to transfer example diversity~\cite{DTN}. Also, to the best of our knowledge, we are the first to propose generating \emph{tensor features} instead of vector features in the few-shot setting.



%These methods in general attempt to either train a generator or identify a way to augment the few-shot dataset during inference in time such that the classification performance is improved. However most of the proposed data augmentation techniques use sophisticated generators borrowed from the general deep learning literature. For example \cite{AFHN} trains a wGAN based feature hallucinator combined with two regularizer while \cite{VIFSL} trains a VAE model where the few labelled examples are used to infer the mean and variance of each class. \cite{DTN} to  transfer  latent  diversities  in order to combine them with support features to generate new features, \cite{Ideme} train a deformation network to fuse reference images with novel images. However, most of these methods follow sophisticated training regimes, such as training a wGAN, VAE, sampling reference images in order to train a generator successfully. In contrast in our work we simply show that using a very simple loss function is more than enough to train a feature hallucinator showing at the same time that there is no added benefit from using any complex training regime.

%Our contributions are summarized below:
%\begin{itemize}
%    \item We show that using a very simple loss function to train a feature hallucinator provides similar performance to sophisticated training regimes such as wGANs and VAEs.
%    \item To the best of our knowledge, we are the first to  propose to generate feature tensors instead of vector features in the few-shot setting, thus exploiting the spatial and structural properties of the feature tensors.
%    \item We achieve new state of the art results comparing all \emph{few-shot} data augmentation techniques.
%    \item We show that our method can be combined with other methods successfully
%\end{itemize}

==> tex/method-1.tex <==
\section{Method}
\label{sec:method}
\subsection{Problem formulation}
\label{sec:problem}

% Following the recent insights from~\cite{rfs}, we follow their formulation for the pre-training stage.

We assume access to a labelled dataset $D_{\base}$ with each example having a label in one of the classes in $C_{\base}$. This dataset is used to learn a parametrized mapping $f_{\theta}: \cX \to \real^d$ from an input space $\cX$ to a $d$-dimensional \emph{feature} or \emph{embedding} space. The knowledge acquired at representation learning is used to solve \emph{novel tasks}, assuming access to a dataset $D_{\novel}$ with each example being associated with one of the classes $C_{\novel}$, where $C_{\novel}$ is disjoint from $C_{\base}$. In \emph{few-shot classification}~\cite{matchingNets}, a novel task is defined by sampling a \emph{support set} $S$ from $D_{\novel}$, consisting of $N$ classes with $K$ labeled examples per class, for a total of $L \defn NK$ examples. Given the mapping $f$ and the support set $S$, the problem is to learn an $N$-way classifier that makes predictions on unlabeled \emph{queries} also sampled from $D_{\novel}$. 
% This may involve adapting $f$ or not. However, $K$ is small and the challenge is to avoid overfitting $S$. 
Queries are treated independently of each other, this is referred to as \emph{inductive inference}.

\subsection{Representation learning}
\label{sec:representation}
The goal of the \emph{representation learning} stage is to learn an embebbing model, $f_{\theta}$, that is transferable and can be applied to $D_{\novel}$ in order to extract expressive vector feature embeddings, $f_{\theta}^{GAP}: \cX \to \real^d$. The use of the superscript term $GAP$ represents global average pooling applied to the output tensors of the backbone network. We follow the recent training regime proposed from \cite{rfs} to train our embedding model and follow a two-stage training regime.
In the first stage, we train the embedding model, $f_{\theta}$, on dataset $D_{\base}$ using standard cross-entropy multi-class classification loss. In order to convert the extracted feature vectors to cross-entropy loss, we use a base classifier, $C_{\phi}$. The complete training loss for the first training stage is defined as:
\begin{equation}
    \{\theta, \phi \} = \arg\min_{\theta, \phi}\displaystyle\sum_{i = 1}^I L^{ce}_i(C_{\phi}(f_{\theta}^{GAP}(x_i)), y_i) + R(\phi)
\label{eq:cls}
\end{equation}

where $R$ is a regularization term, $L^{ce}$ is the standard cross-entropy loss term and $I$ is the total number of available samples in $D_{\base}$. In the second stage of the training regime, we adopt a self-distillation procedure, which is a form of knowledge distillation where the student and teacher models are identical in architecture. The trained embedding model from the first training stage serves as the teacher model and we distill the knowledge from it  into a new student model. The student model is trained using a weighted sum of: a) a cross-entropy loss between the predictions of the student model and the ground truth labels b) a Kullback-Leibler (KL) divergence term between the predictions of the student and the teacher models. The training loss for the second training stage is defined as:
\begin{equation}
    \theta' = \arg\min_{\theta'}\displaystyle\sum_{i = 1}^I(\alpha L^{ce}_i(C_{\phi'}(f_{\theta'}^{GAP}(x_i)), y_i) + R(\phi') + \beta KL(f_{\theta'}^{GAP}(x_i), f_{\theta}^{GAP}(x_i))
\label{eq:kl}
\end{equation}

where $\alpha$ and $\beta$ are scalar weights, $L^{ce}$ is the standard cross-entropy loss, $I$ is the total number of available samples in $D_{\base}$ and $KL$ is the KL divergence of the predictions between the student model, $f_{\theta'}$, and the teacher model, $f_{\theta}$. Also, $C_{\phi'}$ represents an untrained classifier and not the one trained at the first training stage.
\subsection{Feature tensor hallucinator}
We use the student model, $f_{\theta'}$, pre-trained using equation \ref{eq:kl} as our embedding network in order to train our tensor feature hallucinator.
The output from the embedding network is a tensor, $f_{\theta'}: \cX \to \real^{d\times h \times w}$, where $(d, h, w )$ represent the number of channels, height and width of the output tensor. %The most common procedure is to either flatten the tensor or use global average pooling and decrease the dimension to $\real^d$ as it was the case when we trained our embedding model in section \ref{sec:representation}.
All of the existing feature hallucination methods are trained using vector features, however this means that the vector features lose significant information of their spatial and structural properties. In contrast our tensor feature hallucinator is trained on the output tensors before global average pooling is applied and generates tensor features as well. Generating tensors instead of vectors provides the opportunity to use architectures such as convolutional layers to exploit the spatial and structural properties of tensors.

Our tensor feature hallucinator consists of two network modules: a conditioner network, $h_c$, and a generator network, $h_g$. The conditioner network's purpose is to leverage the prototype tensor of each class in order to aid the generator network to generate class-dependent samples. The prototype tensor of every class, $i$, which is used as the input to the conditioner is calculated by:
\begin{equation}
    p_i = \frac{1}{K}\displaystyle\sum_{j=1}^{K}f_{\theta'}(x_i^j)
\label{eq:proto}
\end{equation}
where $p_i$ is the prototype of class $i$ and $K$ is the total number of samples of class $i$. The output is simply a learnt mapping from the prototype tensor to the prototype class-conditional vector, $s_i = h_c(p_i)$. The generator network takes as input a sample from a Normal distribution, $z \sim \mathcal{N}(0, 1)$ and the output of the conditioner network, $s_i$, generating a class-conditional tensor feature from class $i$, $t_i = h_g(z, s_i)$.

\subsection{Training hallucinator}
We train our hallucinator using a meta-training regime in a similar way to \cite{AFHN, semanticAugmentation, deltaencoder}, training over a large number of few-shot episodes. At every iteration we sample a new episode where we randomly sample $N$ different classes from $D_{\base}$ and $K$ samples per class. We calculate the prototype of each class as defined from equation \ref{eq:proto} and pass it to the conditioner network to generate the prototype class-conditional vector $s_i$. We sample $M$ samples from a Normal distribution, $[z^m]^M_{m=1} \sim \mathcal{N}(0, 1)$. Using the $M$ samples and each prototype class-conditional vector $s_i$, we leverage our generator network to generate $M$ conditional tensor features per class $i$,  $[h_g(z^m, s_i)]_{m=1}^M$. We train our tensor hallucinator with the objective to minimize the mean squared error  (MSE) of all class conditional generated samples of class $i$, to their respective class prototype $p_i$ as defined below:
\begin{equation}
    \{c, g\} = \arg \min_{c, g} \frac{1}{MN}\displaystyle\sum_{i = 1}^N\displaystyle\sum_{m=1}^M (h_g(z^m, s_i) - p_i)^2
\end{equation}
where $N$ is the total number of classes per episode and $M$ the number of generated samples per class.
%\begin{equation}
%    \mathbf{V_i} = h_g(\mathbf{Z_i}, s_i)
%\label{eq:vi}
%\end{equation}
%where $\mathbf{V_i}$ are the $M$ generated samples of class $i$, $\mathbf{V_i} = [f_g(z^1_i, s_i), f_g(z^2_i, s_i), \dots, f_g(z^M_i, s_i)]$




\subsection{Few-shot classification}
At inference time, given a few-shot learning task with a support set, $S$, of $N$ unique classes with $K$ examples per class we calculate the tensor feature of each sample using our trained backbone network, $f_{\theta'}$. Using the tensor features we calculate the prototype, $p_i$, of every class $i$ as defined from equation \ref{eq:proto} and using our trained tensor feature hallucinator we generate $M$ class-conditioned samples for every class. We augment the support set, $S$, by combining all the support samples with the generated samples, therefore for each class we have $\{K+M\}$ support samples. We apply global average pooling to both augmented support tensor features and query tensor features and calculate the vector class prototypes using the augmented support set. Lastly we classify each query simply to the class that its class prototype is closer. At inference time, we use vector instead of tensor features to classify queries since experimentally the performance was superior.%It should be noted that at the last stage of he few-shot classification procedure we used vector features instead of tensors for classifying the query samples since experimentally the performance was superior.% and re-calculate the class prototypes using the augmented support set. %Lastly for every query sample we calculate its tensor feature, apply global averaging pooling to both the query tensor feature and the class prototypes and classify the query simply to the class that its class prototype is closer. Note that at inference time rather than calculating each query using its feature tensor and the tensor prototypes, we perform global average pooling since there is negligible difference in classification performance.


==> tex/plots-ext.tex <==
%------------------------------------------------------------------------------
% hack for CVPR style
\makeatletter
\@namedef{ver@everyshi.sty}{}
\makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikzextern}
\usepackage{pgffor}

%------------------------------------------------------------------------------
% externalization
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/related-1.tex <==
\section{Related work}
\label{related}
\subsection{Few-shot learning}
Few-shot learning methods attempt to recognize query examples from novel classes given only a limited amount of labelled examples. One of the most widely researched directions to address few-shot learning is \emph{meta-learning}. Meta-learning approaches can further be partitioned in three different subcategories. \emph{Optimization-based} meta-learning, which aims to learn how to update the learner's meta-parameters~\cite{MAML, CAVIA, reptile, ravilstm}. \cite{MAML, reptile} proposed to train a model for fast adaptation where the model's meta-parameters are updated using simple gradient descent algorithms. \cite{ravilstm} proposed to learn an LSTM-based meta-learner that learns the optimization procedure replacing the standard gradient descent. \emph{Metric-based} meta-learning, which aims to learn a discriminative embedding space where novel examples are easy to classify~\cite{siamese, prototypical, relationnet, matchingNets}. \cite{prototypical} proposed to calculate class prototypes and classify queries to the nearest class prototype. \cite{siamese} proposed to use Siamese networks to compare the similarity between samples while \cite{relationnet} proposed to learn a distance function through the use of a neural network to calculate the similarity between samples. Lastly \emph{model-based} meta-learning, which leverages specific model architectures to learn how to update the learner's parameters effectively. \cite{santoro} proposed to use memory-augmented neural networks to rapidly learn novel information given only few labelled samples while \cite{metaNet} proposed a novel network architecture for rapid generalization. 

Apart from meta-learning, another significant line of research that addresses few-shot learning is \emph{transfer-learning}. Instead of using an episodic training regime that is commonly used in meta-learning methods, transfer-learning approaches leverage training techniques to pre-train a backbone network on a dataset consisting of examples from base classes before adapting the pre-trained network to recognize novel classes. \cite{closerlook} provided insights showing that learning a good feature representation can provide performance on par with the state of the art meta-learning algorithms. %\cite{imprintedweights} proposed to imprint classifier weights by setting them equal to the average feature representation of each class calculated from the novel support examples. 
\cite{manifoldmixup} proposed to train a backbone network combining manifold mixup regularization \cite{man_mixup_or}, self-supervision techniques \cite{gidarisRot} along with the standard cross-entropy loss. \cite{rfs} trained a backbone network by combining standard cross-entropy loss along with self-distillation. \cite{denseclassification} showed that training with dense classification loss before performing global average pooling on the output of the embedding network can aid the training of the embedding network to learn better feature representations.

Beyond \emph{meta-learning} and \emph{transfer learning} approaches, other techniques have been proposed to address the few-shot learning problem. Some approaches attempt to exploit the \emph{manifold structure} of the data. \cite{fewshotGNN1, fewshotGNN2} proposed to use graph neural networks, \cite{embeddingpropagation} proposed to use an embedding propagation module to update the query features leveraging the manifold structure of the support features, \cite{ilpc} proposed to combine label propagation along with label cleaning to iteratively select the query features that are most likely classified correctly. \emph{Domain adaptation} methods such as ~\cite{domain_one, l2cluster} attempt to reduce the domain shift between source and target.  Other methods propose different ways of adapting the feature embeddings, for example \cite{feat} proposed to learn set-to-set functions adapting the support and query samples such that they are more discriminative. \cite{tapnet} proposed task-adaptive projections while \cite{categorytraversalFSL} proposed to identify and use the most relevant feature dimensions. Lastly another promising line of research focuses on \emph{synthetic data generation} methods that propose methods to augment the support set. Our work falls in this category of methods and further elaboration of prior literature in synthetic data generation for few-shot learning can be found in section \ref{sec:fsl_data_aug}.

\subsection{Synthetic data generation}
Generating synthetic data has been at the front line of machine learning and computer vision research in the last few years. The primary interest in generative models is to model the complex underlying data distribution of the training datasets. Multiple different types of generative models have been proposed with generative adversarial networks (GAN) being by far the most researched \cite{GANSgoodfellow}. The main idea behind GANS is to train the generator by setting up a zero-sum game with the discriminator in order to learn how to generate realistic data. Since the initial idea, a lot of improvements have been proposed such as novel generator architectures, better regularization and training techniques \cite{stylegan, biggan, pggan}. Other approaches beyond GANS include variational autoencoders (VAE) that attempt to impose a prior distribution in a lower dimensional latent space such that when sampling a sample in latent space a decoder will decode a realistic data sample \cite{VAE}, autoregressive (AR) models \cite{pixelCNN, condpixelCNN} where they define a distribution through the use of chain rule for conditional probability where at every step the probability of the next step is conditioned on all the previous steps and flow-based models \cite{glow, flow++} that leverage invertible transformations to learn the explicit data distribution.

Even though research in generating synthetic data is vast, most state of the art generative models do not focus on improving the performance of downstream tasks such as classification performance but focus on other metrics such as FID ~\cite{FID} and \cite{IS}. Also often these models assume access to abundance of training data which is in direct contrast to the few-shot learning setting. Even though recent work in generative modeling
tackled the problem of generating images from small datasets \cite{styleganADA, few-shotGAN} these methods focus on unconditional image generation and it is unclear how they can aid classification performance in few-shot learning.

\subsection{Synthetic data generation for few-shot learning}
\label{sec:fsl_data_aug}
The idea of synthetic data generation to augment datasets with small number of samples is an attractive idea. One of the first ideas in this line of research \cite{lowshot2} proposed a novel method to hallucinate embedding features. \cite{dataAG, metaGAN} proposed to integrate meta-learning methods such as MAML \cite{MAML} with a conditional generative adversarial network to generate samples from novel classes to augment the support set. \cite{AFHN} builds on the direction of using GANs as few-shot generative models and proposed to train a GAN-based feature hallucinator using wGAN\cite{wGAN} training loss combined with two regularizers.  \cite{funit} proposed a GAN-based method for few-shot image-to-image translation that also provided good result in few-shot classification. Instead of using GANs, \cite{VIFSL} proposed a novel class-conditional variational autoencoder as a feature hallucinator. \cite{DTN} proposed to train a diversity transfer network to learn how to transfer latent diversities from base classes and apply them to novel class support features to generate novel features. \cite{salnetFSL} proposed to hallucinate novel features by leveraging a saliency network to obtain the foregrounds and backgrounds of available samples. \cite{Ideme} proposed a method to synthesize new examples from novel classes by using a deformation network that learns to deform images by fusing a support example and an image sampled from the training set.

Our work is inspired from the main direction in few-shot synthetic data generation techniques that focuses in generating samples in the feature space rather than in the image space. However in contrast to the rest of the methods we are the first to train a generative model to generate tensor features instead of vector features exploiting the spatial and structural properties of tensors in the process. More importantly we show that using a simple loss function to train our generative model can provide significant performance improvements challenging other approaches using overly complex generative models.

%Multiple different lines of research have been proposed over the years to address the few-shot learning problem. One of the more common lines of research is meta-learning, where they tackle the problem of few-shot learning by the concept of "learning to learn" leveraging training episodes that mimic the few-shot task by having small number of classes and limited number of samples per class. Meta-learning approaches can further be partitioned in optimization-based approaches that attempt to learn to update the learner's model meta-parameters \cite{MAML, CAVIA, reptile, ravilstm}, metric-based approaches that attempt to learn a discriminative embedding space where samples from a novel task are easy to classify \cite{siamese, prototypical, relationnet, matchingNets} and model-based approaches that depend on specific model architectures to learn how to update the learner's parameters effectively \cite{santoro, metaNet}.
%Beyond meta-learning methods, other approaches include methods that leverage the manifold structure of the data either by label propagation or embedding propagation or through the use of graph neural networks \cite{fewshotGNN1, fewshotGNN2, tpn, ilpc} and domain adaptation techniques that attempt to reduce the domain shifts between source and target domain domains \cite{domain_one, l2cluster}. Another line of research constitutes of data augmentation methods that attempt to tackle the data deficiency by effectively providing more training data \cite{AFHN, VIFSL, semanticAugmentation, Ideme, antoniou, metaGAN}.
